Scaling RIFT 1: Extending RIFT to third-generation gravitational-wave analyses

Interpretation of compact binary signals observed by third-generation gravitational-wave detectors is complicated by their high signal-to-noise ratios, often reaching hundreds to thousands, and by time- and frequency-dependent detector responses arising from Earth's rotation and the detectors' large physical extent. Building on prior work for LISA, we implement generic, robust extensions of the RIFT parameter estimation pipeline that enable interpretation of these sources using any existing waveform model, without recourse to intermediate pretrained data products like reduced-order approximations or normalizing flows. We demonstrate end-to-end recovery of finite-size binary-neutron-star injections in a three-site next-generation network to $\mathrm{SNR}=1000$, localizing the source's extrinsic parameters to $0.8\times10^{-3}\,\mathrm{deg}^2$ in minutes on a single GPU.

==> figures/jax_sky_revisit_time_table.tex <==
stored-sample Simpson & finite-sinc & 8192 & 625.434 & --- \\
full-window reconstruction & finite-sinc & 8192 & 4.728 & --- \\
full-window reconstruction & finite-sinc & 16384 & 0.0177 & --- \\
full-window reconstruction & finite-sinc & 32768 & 0.00591 & --- \\
full-window reconstruction & finite-sinc & 65536 & 0.00283 & 9.788\% \\
full-window reconstruction & four-point cubic & 16384 & 0.0431 & --- \\
full-window reconstruction & four-point cubic & 32768 & 0.00261 & 0.037\% \\

